Ensembling Finetuned Language Models for Text Classification

Finetuning is a common practice widespread across different communities to adapt pretrained models to particular tasks. Text classification is one of these tasks for which many pretrained models are available. On the other hand, ensembles of neural networks are typically used to boost performance and provide reliable uncertainty estimates. However, ensembling pretrained models for text classification is not a well-studied avenue. In this paper, we present a metadataset with predictions from five large finetuned models on six datasets, and report results of different ensembling strategies from these predictions. Our results shed light on how ensembling can improve the performance of finetuned text classifiers and incentivize future adoption of ensembles in such tasks.

==> tables/error_ensemblers/ranked.tex <==
\begin{tabular}{lllllllllllll}
\toprule
 & \bfseries 0-RQ1_ftc_extended_error & \bfseries 0-RQ1_ftc_mini_error & \bfseries 1-RQ1_ftc_extended_error & \bfseries 1-RQ1_ftc_mini_error & \bfseries 2-RQ1_ftc_extended_error & \bfseries 2-RQ1_ftc_mini_error & \bfseries 3-RQ1_ftc_extended_error & \bfseries 3-RQ1_ftc_mini_error & \bfseries 4-RQ1_ftc_extended_error & \bfseries 4-RQ1_ftc_mini_error & \bfseries 5-RQ1_ftc_extended_error & \bfseries 5-RQ1_ftc_mini_error \\
\midrule
\bfseries Single-Best & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 \\
\bfseries Random5 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 6.0000 & 7.0000 & 7.0000 & 6.0000 & 7.0000 & 7.0000 & 7.0000 \\
\bfseries Random50 & 6.0000 & 4.0000 & 6.0000 & 6.0000 & 5.0000 & 7.0000 & 6.0000 & 6.0000 & 4.0000 & 4.0000 & 5.0000 & 6.0000 \\
\bfseries Top5 & 3.0000 & 2.0000 & 1.0000 & 3.0000 & 2.5000 & 3.0000 & 1.0000 & 3.0000 & 5.0000 & 6.0000 & 3.0000 & 1.0000 \\
\bfseries Top50 & 5.0000 & 5.0000 & 4.0000 & 4.0000 & 6.0000 & 5.0000 & 4.0000 & 4.0000 & 2.0000 & 5.0000 & 4.0000 & 4.0000 \\
\bfseries Greedy5 & 1.0000 & 3.0000 & 2.5000 & 2.0000 & 2.5000 & 2.0000 & 3.0000 & 1.0000 & 7.0000 & 2.0000 & 1.5000 & 2.0000 \\
\bfseries Greedy50 & 2.0000 & 1.0000 & 2.5000 & 1.0000 & 1.0000 & 1.0000 & 2.0000 & 2.0000 & 1.0000 & 1.0000 & 1.5000 & 3.0000 \\
\bfseries Model Average & 4.0000 & 6.0000 & 5.0000 & 5.0000 & 4.0000 & 4.0000 & 5.0000 & 5.0000 & 3.0000 & 3.0000 & 6.0000 & 5.0000 \\
\bottomrule
\end{tabular}


==> tables/extended_error_ensemblers/aggregated.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Random5 & 0.9253 & 0.2006 & 0.7009 & 0.7258 & 0.4163 & 0.8237 \\
\bfseries Random50 & 0.7329 & 0.1951 & 0.5780 & 0.7084 & 0.4104 & 0.6301 \\
\bfseries Top5 & 0.5032 & 0.1592 & 0.5428 & 0.4809 & 0.4155 & 0.5334 \\
\bfseries Top50 & 0.7320 & 0.1836 & 0.5849 & 0.5505 & 0.4075 & 0.6010 \\
\bfseries Greedy50 & 0.5019 & 0.1606 & 0.5413 & 0.5070 & 0.4042 & 0.5217 \\
\bfseries Model Average & 0.5794 & 0.1865 & 0.5576 & 0.5944 & 0.4085 & 0.6370 \\
\bottomrule
\end{tabular}


==> tables/extended_error_ensemblers/ranked.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 \\
\bfseries Random5 & 6.0000 & 6.0000 & 6.0000 & 6.0000 & 6.0000 & 6.0000 \\
\bfseries Random50 & 5.0000 & 5.0000 & 4.0000 & 5.0000 & 4.0000 & 4.0000 \\
\bfseries Top5 & 2.0000 & 1.0000 & 2.0000 & 1.0000 & 5.0000 & 2.0000 \\
\bfseries Top50 & 4.0000 & 3.0000 & 5.0000 & 3.0000 & 2.0000 & 3.0000 \\
\bfseries Greedy50 & 1.0000 & 2.0000 & 1.0000 & 2.0000 & 1.0000 & 1.0000 \\
\bfseries Model Average & 3.0000 & 4.0000 & 3.0000 & 4.0000 & 3.0000 & 5.0000 \\
\bottomrule
\end{tabular}


==> tables/extended_nll_ensemblers/aggregated.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Random5 & 0.8377 & 0.8093 & 0.8513 & 0.7845 & 0.6588 & 0.8919 \\
\bfseries Random50 & 0.6403 & 0.9176 & 0.6456 & 0.9137 & 0.6299 & 1.0878 \\
\bfseries Top5 & 0.5514 & 0.2844 & 0.6885 & 0.3890 & 0.5671 & 0.3726 \\
\bfseries Top50 & 0.6303 & 0.2889 & 0.6714 & 0.3379 & 0.5047 & 0.3681 \\
\bfseries Greedy50 & 0.4664 & 0.2544 & 0.5078 & 0.3094 & 0.4649 & 0.3219 \\
\bfseries Model Average & 0.5631 & 0.3957 & 0.5317 & 0.4465 & 0.5010 & 0.4875 \\
\bottomrule
\end{tabular}


==> tables/extended_nll_ensemblers/ranked.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 6.0000 \\
\bfseries Random5 & 6.0000 & 5.0000 & 6.0000 & 5.0000 & 6.0000 & 5.0000 \\
\bfseries Random50 & 5.0000 & 6.0000 & 3.0000 & 6.0000 & 5.0000 & 7.0000 \\
\bfseries Top5 & 2.0000 & 2.0000 & 5.0000 & 3.0000 & 4.0000 & 3.0000 \\
\bfseries Top50 & 4.0000 & 3.0000 & 4.0000 & 2.0000 & 3.0000 & 2.0000 \\
\bfseries Greedy50 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Model Average & 3.0000 & 4.0000 & 2.0000 & 4.0000 & 2.0000 & 4.0000 \\
\bottomrule
\end{tabular}


==> tables/mini_error_ensemblers/aggregated.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Random5 & 0.4977 & 0.1580 & 0.3319 & 0.9902 & 0.4702 & 0.7821 \\
\bfseries Random50 & 0.0130 & 0.1491 & 0.3349 & 0.6385 & 0.4507 & 0.5921 \\
\bfseries Top5 & 0.0121 & 0.1205 & 0.2610 & 0.4559 & 0.4607 & 0.4947 \\
\bfseries Top50 & 0.0131 & 0.1235 & 0.3118 & 0.5071 & 0.4511 & 0.5313 \\
\bfseries Greedy50 & 0.0120 & 0.1125 & 0.2544 & 0.4421 & 0.4317 & 0.4999 \\
\bfseries Model Average & 0.0137 & 0.1332 & 0.2963 & 0.5264 & 0.4438 & 0.5764 \\
\bottomrule
\end{tabular}


==> tables/mini_error_ensemblers/ranked.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 \\
\bfseries Random5 & 6.0000 & 6.0000 & 5.0000 & 6.0000 & 6.0000 & 6.0000 \\
\bfseries Random50 & 3.0000 & 5.0000 & 6.0000 & 5.0000 & 3.0000 & 5.0000 \\
\bfseries Top5 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 5.0000 & 1.0000 \\
\bfseries Top50 & 4.0000 & 3.0000 & 4.0000 & 3.0000 & 4.0000 & 3.0000 \\
\bfseries Greedy50 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 2.0000 \\
\bfseries Model Average & 5.0000 & 4.0000 & 3.0000 & 4.0000 & 2.0000 & 4.0000 \\
\bottomrule
\end{tabular}


==> tables/mini_model_comparion.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & imdb & mteb/tweet_sentiment_extraction & ag_news & dbpedia_14 & stanfordnlp/sst2 & SetFit/mnli \\
\midrule
gpt2 & 0.081720 & NaN & 0.073684 & 0.010371 & 0.117483 & 0.238839 \\
bert-large-uncased & 0.075240 & 0.236559 & 0.077237 & 0.008529 & 0.080921 & 0.200738 \\
albert-large-v2 & 0.065040 & 0.243916 & 0.080789 & 0.010543 & 0.091778 & 0.190171 \\
facebook/bart-large & 0.045960 & 0.230617 & 0.065658 & NaN & 0.065423 & 0.133767 \\
google-t5/t5-large & 0.045520 & 0.230334 & 0.073553 & NaN & 0.050668 & NaN \\
\bottomrule
\end{tabular}


==> tables/mini_nll_ensemblers/aggregated.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Random5 & 0.5873 & 0.4143 & 0.6527 & 0.7178 & 0.6013 & 0.6560 \\
\bfseries Random50 & 0.2140 & 0.3767 & 0.6472 & 0.6631 & 0.6186 & 0.7636 \\
\bfseries Top5 & 0.0293 & 0.2231 & 0.4974 & 0.3780 & 0.6294 & 0.3390 \\
\bfseries Top50 & 0.1292 & 0.2162 & 0.6417 & 0.3562 & 0.6440 & 0.2838 \\
\bfseries Greedy50 & 0.0199 & 0.1821 & 0.3593 & 0.2389 & 0.4526 & 0.2669 \\
\bfseries Model Average & 0.0797 & 0.2535 & 0.4629 & 0.3478 & 0.4982 & 0.3689 \\
\bottomrule
\end{tabular}


==> tables/mini_nll_ensemblers/ranked.tex <==
\begin{tabular}{lllllll}
\toprule
 & \bfseries 0 & \bfseries 1 & \bfseries 2 & \bfseries 3 & \bfseries 4 & \bfseries 5 \\
\midrule
\bfseries Single-Best & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 \\
\bfseries Random5 & 6.0000 & 6.0000 & 6.0000 & 6.0000 & 3.0000 & 5.0000 \\
\bfseries Random50 & 5.0000 & 5.0000 & 5.0000 & 5.0000 & 4.0000 & 6.0000 \\
\bfseries Top5 & 2.0000 & 3.0000 & 3.0000 & 4.0000 & 5.0000 & 3.0000 \\
\bfseries Top50 & 4.0000 & 2.0000 & 4.0000 & 3.0000 & 6.0000 & 2.0000 \\
\bfseries Greedy50 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Model Average & 3.0000 & 4.0000 & 2.0000 & 2.0000 & 2.0000 & 4.0000 \\
\bottomrule
\end{tabular}


==> tables/model_comparison.tex <==
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}[3]{*}{\bfseries Method} & \multicolumn{2}{c}{\bfseries DBpedia} & \multicolumn{2}{c}{\bfseries  News } & \multicolumn{2}{c}{\bfseries Set-Fit} & \multicolumn{2}{c}{\bfseries SST2} & \multicolumn{2}{c}{\bfseries Tweet } & \multicolumn{2}{c}{\bfseries IMDB } \\
\cmidrule(rl){2-7} \cmidrule(lr){8-13}
 & \bfseries 100 \% & \bfseries 10 \%  & \bfseries 100 \%  & \bfseries 10 \%  & \bfseries 100 \%  & \bfseries 10 \%  & \bfseries 100 \%  & \bfseries 10 \%  & \bfseries 100 \%  & \bfseries 10 \%  & \bfseries 100 \%  & \bfseries 10 \%  \\
\midrule

\bfseries GPT2 & \bfseries0.0077   & 0.0103    &  0.0611   & 0.0736  & \bfseries0.1898 & 0.2388  & 0.0840  & 0.1174  & -             & -      & 0.0576 & 0.0817  \\
\bfseries Bert-Large & -         & \bfseries 0.0085  & 0.0540    &  0.0772 & - & 0.2007  & 0.0516 & 0.0809  & 0.2031    & 0.2365 & 0.0540 & 0.0752 \\
\bfseries Albert-Large & -         & 0.0105    & 0.0553     & 0.0807  & - & 0.1901  & 0.0513 & 0.0917  & 0.2043     & 0.2439 & 0.0534 & 0.0650  \\
\bfseries Bart-Large & -        & -         & \bfseries 0.0461    & \bfseries0.0656 & - & \bfseries 0.1337 & 0.0482 & 0.0654  & 0.2011     & 0.2306 & \bfseries 0.0342 & 0.0459 \\
\bfseries T5-Large & -       & -         & -           & 0.0735    & - & -  & \bfseries 0.0396&  \bfseries0.0506  & \bfseries 0.1972  & \bfseries 0.2303 & 0.0362  & \bfseries 0.0455  \\
\bottomrule
\end{tabular}


==> tables/nll_ensemblers/ranked.tex <==
\begin{tabular}{lllllllllllll}
\toprule
 & \bfseries 0-RQ1_ftc_extended_nll & \bfseries 0-RQ1_ftc_mini_nll & \bfseries 1-RQ1_ftc_extended_nll & \bfseries 1-RQ1_ftc_mini_nll & \bfseries 2-RQ1_ftc_extended_nll & \bfseries 2-RQ1_ftc_mini_nll & \bfseries 3-RQ1_ftc_extended_nll & \bfseries 3-RQ1_ftc_mini_nll & \bfseries 4-RQ1_ftc_extended_nll & \bfseries 4-RQ1_ftc_mini_nll & \bfseries 5-RQ1_ftc_extended_nll & \bfseries 5-RQ1_ftc_mini_nll \\
\midrule
\bfseries Single-Best & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 7.0000 & 8.0000 \\
\bfseries Random5 & 7.0000 & 7.0000 & 6.0000 & 7.0000 & 7.0000 & 7.0000 & 6.0000 & 7.0000 & 7.0000 & 4.0000 & 6.0000 & 6.0000 \\
\bfseries Random50 & 6.0000 & 6.0000 & 7.0000 & 6.0000 & 4.0000 & 6.0000 & 7.0000 & 6.0000 & 6.0000 & 5.0000 & 8.0000 & 7.0000 \\
\bfseries Top5 & 3.0000 & 3.0000 & 3.0000 & 4.0000 & 6.0000 & 4.0000 & 4.0000 & 5.0000 & 5.0000 & 6.0000 & 4.0000 & 4.0000 \\
\bfseries Top50 & 5.0000 & 5.0000 & 4.0000 & 3.0000 & 5.0000 & 5.0000 & 2.0000 & 4.0000 & 4.0000 & 7.0000 & 3.0000 & 3.0000 \\
\bfseries Greedy5 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 3.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 \\
\bfseries Greedy50 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Model Average & 4.0000 & 4.0000 & 5.0000 & 5.0000 & 3.0000 & 3.0000 & 5.0000 & 3.0000 & 3.0000 & 3.0000 & 5.0000 & 5.0000 \\
\bottomrule
\end{tabular}


==> tables/nll_ensemblers_old/aggregated.tex <==
\begin{tabular}{lllllllllllll}
\toprule
\multirow{2}[3]{*}{\bfseries Method} & \multicolumn{6}{c}{\bfseries Complete} & \multicolumn{6}{c}{\bfseries Mini (10\%)} \\
\cmidrule(rl){2-7} \cmidrule(lr){8-13}
 & \bfseries IMDB & \bfseries Tweet & \bfseries News & \bfseries DBpedia & \bfseries SST2& \bfseries Set-Fit & \bfseries IMDB & \bfseries Tweet & \bfseries News & \bfseries DBpedia & \bfseries SST2& \bfseries Set-Fit \\
\midrule
\bfseries Single-Best & 0.0768 & 0.6218 & 1.0421 & 0.3773 & 1.0266 & 0.3202 & 1.8225 & 1.0861 & 0.9941 & 0.5712 & 1.1217 & 0.4651 \\
\bfseries Random5 & 0.0644 & 0.5032 & 0.8871 & 0.2959 & 0.6763 & 0.2856 & 1.0705 & 0.4500 & 0.6488 & 0.4100 & 0.6745 & 0.3051 \\
\bfseries Random50 & 0.0492 & 0.5706 & 0.6728 & 0.3447 & 0.6466 & 0.3483 & 0.3900 & 0.4091 & 0.6434 & 0.3788 & 0.6939 & 0.3551 \\
\bfseries Top5 & 0.0424 & 0.1768 & 0.7175 & 0.1468 & 0.5822 & 0.1193 & 0.0534 & 0.2423 & 0.4945 & 0.2159 & 0.7060 & 0.1576 \\
\bfseries Top50 & 0.0484 & 0.1796 & 0.6997 & 0.1275 & 0.5181 & 0.1179 & 0.2355 & 0.2348 & 0.6379 & 0.2034 & 0.7223 & 0.1320 \\
\bfseries Greedy5 & 0.0383 & 0.1751 & 0.5413 & 0.1389 & 0.5085 & 0.1150 & 0.0446 & 0.2319 & 0.4037 & 0.1587 & 0.5419 & 0.1272 \\
\bfseries Greedy50 & 0.0358 & 0.1582 & 0.5292 & 0.1167 & 0.4772 & 0.1031 & 0.0364 & 0.1978 & 0.3572 & 0.1365 & 0.5077 & 0.1241 \\
\bfseries Model Average & 0.0433 & 0.2461 & 0.5541 & 0.1685 & 0.5143 & 0.1561 & 0.1453 & 0.2753 & 0.4602 & 0.1987 & 0.5588 & 0.1716 \\
\bottomrule
\end{tabular}


==> tables/nll_ensemblers_old/ranked.tex <==
\begin{tabular}{lllllllllllll}
\toprule
\multirow{2}[3]{*}{\bfseries Method} & \multicolumn{6}{c}{\bfseries Complete} & \multicolumn{6}{c}{\bfseries Mini (10\%)} \\
\cmidrule(rl){2-7} \cmidrule(lr){8-13}
 & \bfseries IMDB & \bfseries Tweet & \bfseries News & \bfseries DBpedia & \bfseries SST2& \bfseries Set-Fit & \bfseries IMDB & \bfseries Tweet & \bfseries News & \bfseries DBpedia & \bfseries SST2& \bfseries Set-Fit \\
\midrule
\bfseries Single-Best & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 7.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 & 8.0000 \\
\bfseries Random5 & 7.0000 & 6.0000 & 7.0000 & 6.0000 & 7.0000 & 6.0000 & 7.0000 & 7.0000 & 7.0000 & 7.0000 & 4.0000 & 6.0000 \\
\bfseries Random50 & 6.0000 & 7.0000 & 4.0000 & 7.0000 & 6.0000 & 8.0000 & 6.0000 & 6.0000 & 6.0000 & 6.0000 & 5.0000 & 7.0000 \\
\bfseries Top5 & 3.0000 & 3.0000 & 6.0000 & 4.0000 & 5.0000 & 4.0000 & 3.0000 & 4.0000 & 4.0000 & 5.0000 & 6.0000 & 4.0000 \\
\bfseries Top50 & 5.0000 & 4.0000 & 5.0000 & 2.0000 & 4.0000 & 3.0000 & 5.0000 & 3.0000 & 5.0000 & 4.0000 & 7.0000 & 3.0000 \\
\bfseries Greedy5 & 2.0000 & 2.0000 & 2.0000 & 3.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 & 2.0000 \\
\bfseries Greedy50 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 & 1.0000 \\
\bfseries Model Average & 4.0000 & 5.0000 & 3.0000 & 5.0000 & 3.0000 & 5.0000 & 4.0000 & 5.0000 & 3.0000 & 3.0000 & 3.0000 & 5.0000 \\
\bottomrule
\end{tabular}

